The Stability of Rutile Oxides for Oxygen Evolution Catalysis: From Mechanistic Understanding to New Descriptors

Polymer electrolyte water electrolysis is considered as a pivotal technology for green hydrogen production. Iridium dioxide (IrO2) serves as the benchmark electrocatalyst for the anodic oxygen evolution reaction (OER) in these cells. However, the scarcity and cost of iridium drives efforts to find durable and cost-effective replacements or drastically reduce the iridium loading. While ruthenium dioxide (RuO2) offers comparable activity, its practical utility is impacted by its stability being inferior to IrO2. The presented computational study analyzes the metal-oxygen bond strengths in bulk IrO2 and RuO2 to provide insights into the electronic origins of their differing stabilities. Through a comparative analysis of the electronic structure of bulk rutile IrO2, RuO2, and selected MO2 systems, it is able to discriminate the covalent and ionic contributions to the metal-oxygen bond using crystal-orbital-derived electronic descriptors.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
  if (!($root_filename eq $_[0])) {
    system( "latexmk -cd -pdf \"$_[0]\"" );
  }
}
